Revisiting reopened bugs in open source software systems

Reopened bugs can degrade the overall quality of a software system since they require unnecessary rework by developers. Moreover, reopened bugs also lead to a loss of trust in the end-users regarding the quality of the software. Thus, predicting bugs that might be reopened could be extremely helpful for software developers to avoid rework. Prior studies on reopened bug prediction focus only on three open source projects (i.e., Apache, Eclipse, and OpenOffice) to generate insights. We observe that one out of the three projects (i.e., Apache) has a data leak issue -- the bug status of reopened was included as training data to predict reopened bugs. In addition, prior studies used an outdated prediction model pipeline (i.e., with old techniques for constructing a prediction model) to predict reopened bugs. Therefore, we revisit the reopened bugs study on a large scale dataset consisting of 47 projects tracked by JIRA using the modern techniques such as SMOTE, permutation importance together with 7 different machine learning models. We study the reopened bugs using a mixed methods approach (i.e., both quantitative and qualitative study). We find that: 1) After using an updated reopened bug prediction model pipeline, only 34% projects give an acceptable performance with AUC >= 0.7. 2) There are four major reasons for a bug getting reopened, that is, technical (i.e., patch/integration issues), documentation, human (i.e., due to incorrect bug assessment), and reasons not shown in the bug reports. 3) In projects with an acceptable AUC, 94% of the reopened bugs are due to patch issues (i.e., the usage of an incorrect patch) identified before bug reopening. Our study revisits reopened bugs and provides new insights into developer's bug reopening activities.

==> Ankur_workspace.tex <==
Software systems are becoming large and are being used by an ever-increasing number of consumers. 

==> Background.tex <==
In this section, we provide an overview of the bug tracking systems and the bug reopening process.

\subsection{Bug tracking systems} Bug tracking systems manage the various bug fixing activities. Bug tracking systems are used to create bug reports, where reporters can provide essential information about the symptoms and causes of bugs. Developers discuss potential fixes of the bug, update the status of the bug in order for others to track the progress of bug fixing. Bugzilla\footnote{\url{https://www.bugzilla.org/}} and JIRA\footnote{\url{https://www.atlassian.com/software/jira}} are the two commonly used bug tracking systems.

Bugs from both Bugzilla and JIRA were studied in prior work. However, prior studies on reopened bugs used bugs from Bugzilla \citep{shihab2010predicting, shihab2013studying, xia2015automatic, xia2013comparative, mi2016empirical, xuan2014towards}. To the best of our knowledge, no prior work has studied reopened bugs that are tracked by JIRA. For example, Shihab et al. studied reopened bugs in three projects, i.e., Apache, Eclipse, and OpenOffice, which are tracked by Bugzilla. \cite{xia2015automatic} extended Shihab et al.'s study using more advanced techniques and the same Bugzilla dataset. \cite{xia2013comparative} investigated the performance of various classifiers.






\subsection{Process of reopening a bug}
A bug transitions through various statuses in its life cycle \citep{jira_priority_and_resolutions_website}. The relevant statuses are explained below:
\begin{itemize}
  \item \textit{Open:} When a new bug is created, its status is set as \textit{open}.
  \item \textit{In progress:} When a developer starts working on a bug, its status is set as \textit{in progress}.
  \item \textit{Resolved:} When a bug has been resolved, its status is set as \textit{resolved}.
  \item \textit{Closed:} When a bug has been fixed and it will not be worked upon anymore, its status is set as \textit{closed}.
  \item \textit{Reopened:} When a bug is not fixed, it needs to be reopened. Therefore, its status is set as \textit{reopened}.
\end{itemize}



Figure \ref{fig_JIRA_life_cycle} shows a generic life cycle of a bug. Initially, a bug is created and its status is set as \textit{open}. Then the bug is assigned to a developer. When the developer starts working on the bug, the bug status is set as \textit{in progress}. When the bug is resolved, the bug's status is set as \textit{resolved}. The bug is then verified and if the fix is correct then the bug status is set as \textit{closed}. However, a bug can be reopened, and the bug status is set as \textit{reopened}.

\begin{figure}[!ht]
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.7\textwidth]{Figures/Bug_life_cycle.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{A generic workflow of the bug fixing process}
\label{fig_JIRA_life_cycle}       % Give a unique label
\end{figure}

Bug reopening can involve a discussion between developers. For example, in a bug report\footnote{\url{https://issues.apache.org/jira/browse/CXF-6089}} (ID: 6089) for the Apache CXF project, a developer discusses with another developer that \textit{``mmh... reopening as there's a testcase failing, I didn't notice that locally (likely run with -Pfastinstall) Rebecca, please have a look, I might revert the changes in the mean time.''} \citep{cxf_6089_comment_website}. In another example, a developer pointed out in a bug report\footnote{\url{https://issues.apache.org/jira/browse/HAWQ-737}} (ID: 737) for the Apache HAWQ project that the bug will be reopened to update the version \citep{hawq_737_comment_website}.





% Notes

% \hz{your goal is never to predict, is actually to explain why bugs are reopened}

% \h{check Xin's ASE'14 paper page 31, see how they mention a bug} \atagra{I fixed this, also i removed the footnotes for link to bugs, because using the bug id and project name, bug report can be found}


% Bugzilla helps in improving communication among developers. Bugzilla also increases the productivity of the team in bug fixing activity and increase the customer satisfaction\footnote{\url{https://www.bugzilla.org/}}. 


% There are existing studies that use Bugzilla to study duplicate bugs \citep{tian2012improved, jalbert2008automated}. \cite{tian2015automated} predicted the bug priority levels using Bugzilla. \cite{somasundaram2012automatic} studied the categorization of bugs using Bugzilla.


% Bugzilla is a bug tracking system developed by the Mozilla project and released as open-source in 1998\footnote{\url{https://en.wikipedia.org/wiki/Bugzilla}}. JIRA is built to create, manage, and track bugs for software projects\footnote{\url{https://www.atlassian.com/software/jira/bug-tracking}}.  Using JIRA, the development teams can track their bug fixing activities. Prior studies also leverage JIRA in their studies of bugs. For example, \cite{zhou2017automated} used the JIRA dataset in their study to automatically identify security issues. \cite{herzig2013s} studied JIRA bugs to find the impact of misclassification on bug prediction.


% JIRA is a more widely used bug tracking system compared to Bugzilla as a total of 589 projects use JIRA for bug tracking while only 138 projects use Bugzilla\footnote{\url{https://www.bugzilla.org/installation-list/}}. Also, out of 10 popular features \citep{jira_vs_bugzilla} provided by JIRA for software development teams, only three are supported by Bugzilla. For example, JIRA provides kanban boards and real-time release tracking \citep{jira_vs_bugzilla}, while such features are not provided by Bugzilla. Though JIRA hosts more projects and provides more features to the development teams, most of the prior studies focused only on Bugzilla to study reopened bugs \citep{shihab2010predicting, shihab2013studying, xia2015automatic, xia2013comparative, mi2016empirical, xuan2014towards}. To the best of our knowledge, no prior work has studied reopened bugs that are tracked by JIRA. For example, Shihab et al. studied reopened bugs in three projects, i.e., Apache, Eclipse, and OpenOffice, which are tracked by Bugzilla. \cite{xia2015automatic} extended Shihab et al.'s study using more advanced techniques and the same Bugzilla dataset to predict reopened bugs. \cite{xia2013comparative} investigated the performance of various classifiers to predict reopened bugs using Bugzilla dataset. In our study, we study reopened bugs from both Bugzilla and JIRA. More specifically, we firstly replicate the study by Shihab et al. to understand whether a bug tracked by Bugzilla will be reopened, then we collect bugs from JIRA and build classifiers to understand whether a bug tracked by JIRA will be reopened.

==> RQ1.tex <==
%  this is now obsolete



% \textbf{Motivation:} The study to predict reopened bugs was performed seven years before (i.e., in 2013) \citep{shihab2013studying}. A lot of software processes have changed since then and so does the bug reporting process\atagra{which}. The findings \atagra{emad, or which findings} were based on 3 open source projects (i.e., Apache, Eclipse, and OpenOffice). Moreover, when we investigated their dataset we observed that 80.6\% (745/924) reopened bug reports have a feature “last status” which has value as reopened in the apache project. These are flawed bug reports and need to be removed from the analysis of the prediction of reopened bug reports. Therefore, all the prior findings on reopened bugs are based on 2 datasets (i.e., Eclipse and OpenOffice). In this RQ, we investigate if the performance of the reopened bug prediction models fall when we remove the flawed bug reports. 

% link - https://tex.stackexchange.com/questions/48632/underscores-in-words-text

% \noindent \textbf{Approach:} We investigated the prior dataset for reopened bug reports. We computed all the last status which contain a substring “reopened” to determine the flawed bug reports in the dataset. We also manually searched in Bugzilla about the bugs with criteria such as reporter names, components, and hardware as the bug id is not provided in Emad’s bug dataset. We tracked down some of the bugs based on these search criteria. Some of the searches resulted in multiple bug reports, we studied all of them manually, and based on closing month or resolved month or dates we identified matching bug reports. This is a challenging task as not all searches result in the exact mapping of bug reports with the dataset. For example, we identified an Apache bug report that was labeled as ``reopened'' as well as the last status was also reopened. Figure \ref{fig_flawed_bug_report} shows a flawed Apache reopened bug report.

% We remove all the bug reports from the analysis which have the last status as ``Reopened'', and we call this a reduced dataset. We implement the reopened bug prediction model. We execute the prediction model on two types of datasets i.e., whole dataset and reduced dataset. We use the Bugzilla dataset for our analysis. We use the same classifier (i.e. Decision Tree) as used by \cite{shihab2013studying}. We use SMOTE to address class imbalance problems. We also use Grid Search based hyperparameter tuning to improve the performance of the bug prediction model. \cite{shihab2013studying} used top node analysis for computing feature importance. However, we do apply the latest techniques for feature importance such as permutation feature importance, by computing feature importance for each permutation, and then ranking these features based on the Sk\_esd test. We also compare our feature importance results with those shared by \cite{shihab2013studying}. They compute the important features using top node analysis. They consider a feature as most important if it is always the root node. The other important features are on nodes with level 1.  As they go down the levels of the tree, the features become less important. To compare our results with their results. We use their top node analysis results to get the top 5 important features. To generate their top 5 features, we select a feature as most important if its occurrence is maximum at the root node. We then select the next important feature with the second highest count on the root node and so on. If all the features on the root node are selected then we select the feature with the most occurrence on level 1 nodes. If root node and level 1 node features are selected, then we don't select any other feature as they don't provide features on level 2 and subsequent levels on the tree. We then generate a table to compare our results with the results of \cite{shihab2013studying} paper. \\


% \begin{figure}
% \centering
% % Use the relevant command to insert your figure file.
% % For example, with the graphicx package use
%   \includegraphics[width=0.9\textwidth]{Figures/bugzilla_apache_953.pdf}
% % figures can also be resized by adding to the include graphics command as follows
% % \includegraphics[width=1.0\textwidth]{example.eps}
% % figure caption is below the figure
% \caption{Flawed Apache bug report with last status as reopened}
% \label{fig_flawed_bug_report}       % Give a unique label
% \end{figure}



% \atagra{Figures numbers are not correct as per references - pending}

% \begin{figure}
% \centering
% % Use the relevant command to insert your figure file.
% % For example, with the graphicx package use
%   \includegraphics[width=0.9\textwidth]{Figures/last_status_project1.pdf}
% % figures can also be resized by adding to the include graphics command as follows
% % \includegraphics[width=1.0\textwidth]{example.eps}
% % figure caption is below the figure
% \caption{Distribution plot of leaked feature from \cite{shihab2013studying} dataset}
% \label{fig_distribution_plot_last_status_reopened}       % Give a unique label
% \end{figure}

% \begin{figure}
% \centering
% % Use the relevant command to insert your figure file.
% % For example, with the graphicx package use
%   \includegraphics[width=0.7\textwidth]{Figures/plot_Emad_all_vs_reduced_AUC.pdf}
% % figures can also be resized by adding to the include graphics command as follows
% % \includegraphics[width=1.0\textwidth]{example.eps}
% % figure caption is below the figure
% \caption{Reopened bug Prediction AUC for All vs reduced dataset}
% \label{fig_AUC_all_vs_reduced}       % Give a unique label
% \end{figure}

% \noindent \textbf{Results:}  \gopi{0: All the prior findings are based only on 3 projects}\h{1: We can report 2 out of 3 projects we can replicate their results, and 1 project we cannot. 1 project data and auc. 2: talk about feature importance of all three projects.}\atagra{I have fixed this, i generated three results paragraph each with a different finding}\\

% \atagra{1st result}\atagra{Read papers and come up with a strategy} \textbf{We were able to achieve either equal or better performance in replicate \cite{shihab2013studying} study of reopened bug prediction model in 2 out of 3 studied projects (i.e., Apache and Eclipse )}. The prior work  considered ``precision'', ``recall'', ``f1-score'', and ``accuracy'' to measure the performance of their reopened bug prediction model. We also evaluated the same performance measures with an extra AUC performance measure in the replication study. In the Apache project, the precision of the prior work model for predicting reopened bug reports is 52.3\%, whereas while replicating their study the model precision is observed as 67.4\% (i.e., 28.8\% more than in the prior work). Also, the recall for prior work model is  94.1\%, whereas while replicating the prior work, the model recall is observed as 75.5\% (i.e., 19.8\% less than in the prior work). The f1-score for prior work model is  67.2\%, whereas while replicating the prior work, we observed the f1-score as 70.9\% (i.e., 5.5\% more than in the prior work). The accuracy for prior work model is  94\%, while replicating the prior work, we observe the accuracy as 96\% (i.e., 2.1\% more than in prior work).

% In Eclipse project, the precision of the prior work model is  52.1\%, whereas while replicating their study the model precision is observed as 62.2\% (i.e., 19.4\% more than in prior work). The recall for prior work model is  70.5\%, whereas while replicating the prior work, the model recall is observed as 69.7\% (i.e., 1.1\% less than in the prior work). The f1-score for prior work model is 59.4\%, whereas while replicating the prior work, we observed the f1-score as 65.2\% (i.e., 9.8\% more than in the prior work). The accuracy for prior work model is 84.2\%, while replicating the prior work, we observe the accuracy as 88\% (i.e., 4.5\% more than in the prior work).\\
% In the OpenOffice project, the precision of the prior work model for predicting reopened bug reports is 78.6\%, whereas while replicating their study the model precision is observed as 75.5\% (i.e., 3.9\% less than in the prior work). The recall for prior work model is  89.3\%, whereas while replicating the prior work, the model recall is observed as 80.9\% (i.e., 9.4\% less than in the prior work). The f1-score for prior work model is  83.6\%, whereas while replicating the prior work, we observed the f1-score as 77.5\% (i.e., 7.3\% less than in the prior work).The accuracy for prior work model is 90.8\%, while replicating the prior work, we observe the accuracy as 88\% (i.e., 3.1\% less than in the prior work). Overall, the precision, f1-score and accuracy of the reopened bug prediction improves and recall of the model decreases while replicating the prior work in 2 of the 3 projects (i.e., Apache and Eclipse) and all performance parameters (i.e., precision, recall, f1-score and accuracy) decrease while replicating the prediction of reopened bug reports in the OpenOffice project.\atagra{add only accuracy stuff}

% \atagra{2nd result}\atagra{Read papers and come up with a strategy} \textbf{Upon analyzing the prior reopened bug prediction dataset, we observed that 2 out of 3 studied projects (i.e., Apache and OpenOffice) have data leak issues. After addressing the data leak issue, we observe that reopened bug prediction model performance only hold for 2 out of 3 projects (i.e., Eclipse and OpenOffice)}
% We investigated the \cite{shihab2013studying} dataset and we observed that, in the Apache project, there are 8.8\% (i.e., 1,262 out of 14,324) bug reports with a \textit{reopened} last status. More specifically, 80.6\% (i.e., 745 out of the 924) bug reports labelled as reopened have a  last status as \textit{reopened}. In these bug reports, the last status before the first occurrence of bug reopening should not be \textit{reopened}. In addition, 3.9\% (i.e., 517 out of the 13,400) bug reports labelled as non reopened have a last status as \textit{reopened}. In these bug reports the last status should not be \textit{reopened} because a bug report labelled as non reopened can't have a reopened state. Also, in the OpenOffice project, 0.3\%(i.e., 104 out of 40,169) bug reports have the last status as \textit{reopened}. More specifically, 0.4\% (i.e., 39 out of 10,569) bug reports labelled as reopened have their last status as \textit{reopened} and 0.2\% (i.e., 65 out of 29,600) bug reports labelled as non reopened have the last status as \textit{reopened}. However, we did not find any bug report with last status as \textit{reopened} in the Eclipse project. Figure \ref{fig_distribution_plot_last_status_reopened} shows the number of bug reports with the last status as Reopened in the Apache and the OpenOffice projects.\\
% After removing all the flawed bug reports (i.e., bug reports with data leak issues) from the analysis, we found that the performance (i.e., AUC) of reopened bug prediction model on Apache depreciates by 7.1\% (AUC dropped from 0.942 to 0.875). We observed a slight increase of 0.1\% performance (i.e., AUC) after removing flawed bug reports. Eclipse project does not have any flawed bug reports so we did not see a change in performance of the reopened bug prediction model in the Eclipse project. This suggests that the prior performance of reopened bug prediction models only hold for Eclipse and OpenOffice projects. However we cannot draw the same conclusion as \cite{shihab2013studying} in the model performance of the Apache project. Table \ref{table:table_reduced_vs_all_RQ1} shows the performance of the reopened bug prediction model for 3 different scenarios (i.e., \cite{shihab2013studying} performance, replication performance and reduced data performance).

% \atagra{3rd result}\atagra{Read papers and come up with a strategy} \textbf{After addressing the data leak issue, the most important features in predicting reopened bug reports remain consistent in only 2 out of 3 projects (i.e., Eclipse and OpenOffice).} \cite{shihab2013studying} found that \textit{last status} and \textit{description text} are the top two most important features in predicting reopened bug reports, in the Apache project. Whereas we found that \textit{description text} and \textit{comment text} are the top 2 most important features in predicting the reopened bug reports. We observed that in the Apache project, after removing the flawed bug reports (i.e., bug reports with data leak issues) the top two most important features change to \textit{description text} and \textit{description size}. In both the cases (i.e., with all bug reports and with reduced bug reports) we could not find \textit{last status} as the top most important feature in predicting the reopened bug reports.

% In the Eclipse project, we were able to replicate the findings of the prior work, the prior work found that \textit{comment text} and \textit{description text} are the top 2 most important features in predicting the reopened bug reports. We also observed that \textit{comment text} and the \textit{description text} are the top two most important features in predicting the reopened bug reports.

% In the Openoffice project, \cite{shihab2013studying} found that \textit{comment text} and the \textit{last status} are the top two most important features in predicting the reopened bug reports. Whereas we found that \textit{comment text} and the \textit{description text} are the top 2 most important features in predicting the reopened bug reports. Even after removing the flawed bug reports, the top 2 most important features in predicting the reopened bug reports remain consistent.

% We compare the most important features in our analysis, in the 2 scenarios i.e., 1) with all the dataset 2) with the reduced dataset. We observe that in the Apache project only 2 out of top 5 most important features remain consistent in both the scenarios, if we consider the order of importance of the features. If we ignore the order of importance of features, then 3 out of 5 top most important features remain consistent in both the scenarios. In Eclipse and OpenOffice all 5 top most important features remain consistent in the two scenarios. Therefore, we observe that the top most important features remain consistent only in 2 out of 3 projects (i.e., Eclipse and OpenOffice) after addressing the data leak issue.


% \h{do not put a newline break after each paragraph}

% \textbf{Upon addressing the data leak, we were able to replicate Shihab et. al.'s results only on two (i.e., OpenOffice and Eclipse) out of the three studied projects. On the Apache project, we observe a 6\% }
% \h{check} \textbf{In our replicate study to predict reopened bugs based on three projects, we are able to predict reopened bugs in two (i.e., OpenOffice and Eclipse) out of the three projects. However, in the Apache project, we cannot draw the same conclusion by~\cite{shihab2013studying}.} In the OpenOffice and Eclipse project, we achieve the same AUC value of 0.92\atagra{fixed} and 0.85 for predicting reopened bugs as~\cite{shihab2013studying}, respectively. We observe that in the OpenOffice project, 39 (i.e., 0.4\%) of the reopened bugs had their last status before reopening as \textit{reopened}, indicating a data leak issue. In these bug reports, the last status for predicting reopened bugs should not have a value of \textit{reopened} before the first time a bug was identified as a reopened bug. By removing these data points with flaw, the model reaches the same value of AUC due to the small number of such data points.

% \h{check} In the Apache project, there are 1,262 (i.e., 8.8\%) of the data points with a \textit{reopened} last status. More specifically, 745 out of the 924 positive data points (i.e., labeled as reopened bugs) have a \textit{reopened} last status. In these bug reports, the last status before the first occurrence of bug reopening should not be \textit{reopened}. In addition, 517 out of the 13,400 negative data points (i.e., labeled as nonreopened bugs) have a \textit{reopened} last status. After removing these data points, our replicate model has a dropped AUC of 0.88 from the value of 0.94. Therefore, one out of the three studied projects to understand bug reopening activities can not be validated due to the data leak issue. Additional effort is required to better understand the reopened bugs.





% \textbf{AUC drops by \atagra{fixed} 7.1\% for Apache project when flawed bug reports are removed.} We remove the flawed bug reports from the analysis and we recompute the performance of the prediction model. We observe that the maximum drop in AUC of 7.1\% is reported in the Apache project. We did not observe any substantial change in the performance of the OpenOffice project. Figure \ref{fig_AUC_all_vs_reduced} shows the AUC for various projects in all data as well as in the reduced dataset. We observe that\atagra{fixed} for project Apache the new AUC is substantially less than the all data AUC without removing flawed bug reports.

% \atagra{fixed}Table \ref{table:table_reduced_vs_all_RQ1} shows the performance of the reopened bug prediction model for all data vs reduced data. 
% We observe that for the Apache project the precision of Reopened bug report prediction dropped by 43\% (38.4/67.4) and recall for of Reopened bug prediction dropped by 24.6\% (56.9/75.5) and F1 score dropped by 38.6\% (43.5/70.9). The AUC dropped by 7.1\% (87.5/94.2). The accuracy slightly improved by 2\%. There was no substantial change in performance metrics for prediction of non reopened bug reports. The Table \ref{table:ratio_AUC} shows the ratio of performance of reduced vs all dataset.


% \textbf{Last status is no longer the most important feature in predicting reopened bug reports.}
% We observed that after removing the flawed bug reports, description text is the most important feature in predicting reopened bug reports in the Apache project. This also reflects the fact that the last status feature in Apache\atagra{fixed- throughout the paper} had a high amount of flawed bug reports as compared to OpenOffice project.\\
% Table \ref{table:table_feature_importance_RQ1} shows the most important features in predicting reopened bug reports. We compare the most important features for (1) \cite{shihab2013studying} important features (2) our important features in all dataset (3) our important features in reduced dataset.\atagra{fixed} We see that in Apache and OpenOffice projects the top 2 important features in \cite{shihab2013studying} paper include the last status. This is due to the faulty behavior of this feature as we have seen that the ``Last status'' feature has a data leak issue. In our study, we found that the ``description text'' is an important feature instead of the ``Last status''. For the Eclipse project we match exactly the top 2 important features in predicting reopened bug reports by \cite{shihab2013studying}. The third feature as per the top node analysis study is Severity changed whereas we found that priority is the third most important feature. For Apache, we exactly match 2 features with their study with the order of importance. If we ignore importance order then we match 3 features in 5 most important features. For OpenOffice, they only provide 2 important features i.e., ``comment text'' and ``Last status'', we also found that ``comment text'' is the most important feature in the OpenOffice dataset. \cite{shihab2013studying} found in their study that last status and the comment text are the most important features in predicting reopened bug reports. Whereas we identify comments text as well as description text to be the most important features in the reopened bug prediction in 3 Bugzilla projects (Apache, Eclipse, and OpenOffice).

% \h{2020-11-13}

% Replication study:
% Motivation: 1. highlight the data quality (data leak, show example), 2. highlight the new approach (SMOTE, hyper?, citations).
% Results: 1. (pending)(need to figure out how good is our result, then we can decide a sell)
% Results: 2. Important features.

% important features

% \h{2020-11-13}

% \begin{table}[]
% \caption{Model performance all data vs reduced dataset}
% \label{table:table_reduced_vs_all_RQ1}
% \begin{tabular}{|l|r|r|r|r|r|r|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Type of \\ dataset\end{tabular}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}All \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}All \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} & \multicolumn{1}{l|}{All data}                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Project \\ name\end{tabular}     & \multicolumn{1}{l|}{Apache}                                              & \multicolumn{1}{l|}{Apache}                                                  & \multicolumn{1}{l|}{Eclipse}                                             & \multicolumn{1}{l|}{Eclipse}                                                 & \multicolumn{1}{l|}{OpenOffice}                        & \multicolumn{1}{l|}{OpenOffice}                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Precision \\ R\end{tabular}      & \begin{tabular}[c]{@{}r@{}}67.4 \\ (0.55)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}38.4 \\ (1.59)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}62.2 \\ (1.09)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}62.2 \\ (1.09)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}75.5 \\ (0.21)\end{tabular} & \begin{tabular}[c]{@{}r@{}}75.4 \\ (0.21)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}Recall \\ R\end{tabular}         & \begin{tabular}[c]{@{}r@{}}75.5 \\ (0.29)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}56.9 \\ (2)\end{tabular}                          & \begin{tabular}[c]{@{}r@{}}69.7 \\ (0.74)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}69.7 \\ (0.74)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}80.9 \\ (1.91)\end{tabular} & \begin{tabular}[c]{@{}r@{}}80.7 \\ (2.01)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}F1- Score \\ R\end{tabular}      & \begin{tabular}[c]{@{}r@{}}70.9 \\ (0.17)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}43.5 \\ (0.73)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}65.2 \\ (0.61)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}65.2 \\ (0.61)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}77.5 \\ (0.73)\end{tabular} & \begin{tabular}[c]{@{}r@{}}77.3 \\ (0.75)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}Precision \\ NR\end{tabular}     & \begin{tabular}[c]{@{}r@{}}98.3 \\ (0)\end{tabular}                      & \begin{tabular}[c]{@{}r@{}}99.3 \\ (0)\end{tabular}                          & \begin{tabular}[c]{@{}r@{}}94.1 \\ (0.03)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}94.1 \\ (0.03)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}93.2 \\ (0.18)\end{tabular} & \begin{tabular}[c]{@{}r@{}}93.2 \\ (0.19)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}Recall \\ NR\end{tabular}        & \begin{tabular}[c]{@{}r@{}}97.4 \\ (0.01)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}98.5 \\ (0.01)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}91.5 \\ (0.12)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}91.5 \\ (0.12)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}90.6 \\ (0.07)\end{tabular} & \begin{tabular}[c]{@{}r@{}}90.5 \\ (0.07)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}F1-Score \\ NR\end{tabular}      & \begin{tabular}[c]{@{}r@{}}97.9 \\ (0)\end{tabular}                      & \begin{tabular}[c]{@{}r@{}}98.9 \\ (0)\end{tabular}                          & \begin{tabular}[c]{@{}r@{}}92.6 \\ (0.04)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}92.6 \\ (0.04)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}91.8 \\ (0.05)\end{tabular} & \begin{tabular}[c]{@{}r@{}}91.7 \\ (0.04)\end{tabular}                       \\ \hline
% \begin{tabular}[c]{@{}l@{}}Average \\ accuracy\end{tabular} & \begin{tabular}[c]{@{}r@{}}96 \\ (0.01)\end{tabular}                     & \begin{tabular}[c]{@{}r@{}}97.9 \\ (0.01)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}88 \\ (0.11)\end{tabular}                     & \begin{tabular}[c]{@{}r@{}}88 \\ (0.11)\end{tabular}                         & \begin{tabular}[c]{@{}r@{}}88 \\ (0.11)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}88 \\ (0.11)\end{tabular}                         \\ \hline
% AUC                                                         & \begin{tabular}[c]{@{}r@{}}94.2 \\ (0.04)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}87.5 \\ (0.03)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}84.5 \\ (0.22)\end{tabular}                   & \begin{tabular}[c]{@{}r@{}}84.5 \\ (0.22)\end{tabular}                       & \begin{tabular}[c]{@{}r@{}}91.9 \\ (0.19)\end{tabular} & \begin{tabular}[c]{@{}r@{}}92 \\ (0.18)\end{tabular}                         \\ \hline
% \end{tabular}
% \end{table}

% #####################################

% \atagra{table rotate by taking transpose - done}
% \atagra{Table add borders - pending} 




% #########################################
% Table with 3 comparisons shihab, all,reduced

% \begin{table}[]
% \caption{Model performance all data vs reduced dataset}
% \label{table:table_reduced_vs_all_RQ1}
% \Rotatebox{90}{%
% \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Type of \\ dataset\end{tabular}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Shihab \\ et al. data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}All \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Shihab \\ et al. data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}All \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Shihab \\ et al. data\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}All \\ data\end{tabular}}   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reduced \\ data\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Project \\ name\end{tabular}     & \multicolumn{1}{l|}{Apache}                                                        & \multicolumn{1}{l|}{Apache}                                              & \multicolumn{1}{l|}{Apache}                                                  & \multicolumn{1}{l|}{Eclipse}                                                       & \multicolumn{1}{l|}{Eclipse}                                             & \multicolumn{1}{l|}{Eclipse}                                                 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Open\\ Office\end{tabular}}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Open\\ Office\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Open\\ Office\end{tabular}}   \\ \hline
% \begin{tabular}[c]{@{}l@{}}Precision \\ R\end{tabular}      & 52.3(0.09)                                                                         & 67.4 (0.55)                                                              & 38.4 (1.59)                                                                  & 52.1(0.99)                                                                         & 62.2 (1.09)                                                              & 62.2 (1.09)                                                                  & 78.6(0.02)                                                                         & 75.5 (0.21)                                                                & 75.4 (0.21)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Recall \\ R\end{tabular}         & 94.1(0.05)                                                                         & 75.5 (0.29)                                                              & 56.9 (2)                                                                     & 70.5(0.69)                                                                         & 69.7 (0.74)                                                              & 69.7 (0.74)                                                                  & 89.3(0.01)                                                                         & 80.9 (1.91)                                                                & 80.7 (2.01)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}F1- score \\ R\end{tabular}      & 67.2(0.07)                                                                         & 70.9 (0.17)                                                              & 43.5 (0.73)                                                                  & 59.4(0.55)                                                                         & 65.2 (0.61)                                                              & 65.2 (0.61)                                                                  & 83.6(0.01)                                                                         & 77.5 (0.73)                                                                & 77.3 (0.75)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Precision \\ NR\end{tabular}     & 99.6(0.00)                                                                         & 98.3 (0)                                                                 & 99.3 (0)                                                                     & 93.9(0.02)                                                                         & 94.1 (0.03)                                                              & 94.1 (0.03)                                                                  & 95.9(0.00)                                                                         & 93.2 (0.18)                                                                & 93.2 (0.19)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Recall \\ NR\end{tabular}        & 94.1(0.01)                                                                         & 97.4 (0.01)                                                              & 98.5 (0.01)                                                                  & 86.8(0.21)                                                                         & 91.5 (0.12)                                                              & 91.5 (0.12)                                                                  & 91.3(0.01)                                                                         & 90.6 (0.07)                                                                & 90.5 (0.07)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}F1-Score \\ NR\end{tabular}      & 96.7(0.00)                                                                         & 97.9 (0)                                                                 & 98.9 (0)                                                                     & 90.2(0.07)                                                                         & 92.6 (0.04)                                                              & 92.6 (0.04)                                                                  & 93.6(0.00)                                                                         & 91.8 (0.05)                                                                & 91.7 (0.04)                                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Average \\ accuracy\end{tabular} & 94.0(0.00)                                                                         & 96 (0.01)                                                                & 97.9 (0.01)                                                                  & 84.2(0.15)                                                                         & 88 (0.11)                                                                & 88 (0.11)                                                                    & 90.8(0.00)                                                                         & 88 (0.11)                                                                  & 88 (0.11)                                                                    \\ \hline
% AUC                                                         & -                                                                                  & 94.2 (0.04)                                                              & 87.5 (0.03)                                                                  & -                                                                                  & 84.5 (0.22)                                                              & 84.5 (0.22)                                                                  & -                                                                                  & 91.9 (0.19)                                                                & 92 (0.18)                                                                    \\ \hline
% \end{tabular}
% }%
% \end{table}




%  #######################################



%  another table

% \begin{table}[]
% \caption{Ratio of performance, where statistical\atagra{fixed} significance: * p $<$ 0.05, ** p $<$ 0.01, *** p $<$ 0.001}
% \label{table:ratio_AUC}
% \begin{tabular}{|l|r|r|r|}
% \hline
% Project Name           & \multicolumn{1}{l|}{Apache} & \multicolumn{1}{l|}{Eclipse} & \multicolumn{1}{l|}{OpenOffice} \\ \hline
% Ratio Precision R      & 0.57***                     & 1                            & 0.99                            \\ \hline
% Ratio Recall R         & 0.75***                     & 1                            & 0.99                            \\ \hline
% Ratio F1-Score R       & 0.61***                     & 1                            & 0.99                            \\ \hline
% Ratio Precision NR     & 1.01***                     & 1                            & 1                               \\ \hline
% Ratio Recall NR        & 1.01***                     & 1                            & 0.99                            \\ \hline
% Ratio F1-Score NR      & 1.01***                     & 1                            & 0.99                            \\ \hline
% Ratio Average Accuracy & 1.02***                     & 1                            & 1                               \\ \hline
% Ratio AUC              & 0.93***                     & 1                            & 1                               \\ \hline
% \end{tabular}
% \end{table}










% \begin{table}[]
% \caption{Feature Rank in Shihab's data vs our data\h{why this is not addressede?}}
% \label{table:table_feature_importance_RQ1}

% \begin{tabular}{lllll}
% Project     & Rank & Shihab's feature   & Our Feature (reduced data) & Our feature (all data) \\
% Apache      & 1    & Last status        & Description text           & Description text       \\
%             & 2    & Description text   & Description Size           & Comments text          \\
%             & 3    & Comment text       & Comments text              & Description size       \\
%             & 4    & Number of comments & Number of comments         & Number of comments     \\
%             & 5    & Month              & Time days                  & Number of files in fix \\
% Eclipse     & 1    & Comment text       & Comment text               & Comment text           \\
%             & 2    & Description text   & Description text           & Description text       \\
%             & 3    & Severity changed   & Priority                   & Priority               \\
%             & 4    & Time               & description size           & description size       \\
%             & 5    & NA                 & Time days                  & Time days              \\
% Open Office & 1    & Comment text       & Comment text               & Comment text           \\
%             & 2    & Last status        & Description text           & Description text       \\
%             & 3    & NA                 & fixer experience           & fixer experience       \\
%             & 4    & NA                 & Comment size               & Comment size           \\
%             & 5    & NA                 & Time days                  & Time days             
% \end{tabular}
% \end{table}





% \begin{table}[]
% \caption{Feature Rank in \cite{shihab2013studying} data vs our data}
% \label{table:table_feature_importance_RQ1}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Project    & Rank & \cite{shihab2013studying} feature                                              & \begin{tabular}[c]{@{}l@{}}Our Feature \\ (reduced data)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Our feature \\ (all data)\end{tabular} \\ \hline
% Apache     & 1    & Last status                                                   & Description text                                                      & Description text                                                  \\ \hline
%           & 2    & Description text                                              & Description Size                                                      & Comments text                                                     \\ \hline
%           & 3    & Comment text                                                  & Comments text                                                         & Description size                                                  \\ \hline
%           & 4    & \begin{tabular}[c]{@{}l@{}}Number of \\ comments\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of \\ comments\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Number of \\ comments\end{tabular}     \\ \hline
%           & 5    & Month                                                         & Time days                                                             & \begin{tabular}[c]{@{}l@{}}Number of\\  files in fix\end{tabular} \\ \hline
% Eclipse    & 1    & Comment text                                                  & Comment text                                                          & Comment text                                                      \\ \hline
%           & 2    & Description text                                              & Description text                                                      & Description text                                                  \\ \hline
%           & 3    & Severity changed                                              & Priority,                                                             & Priority                                                          \\ \hline
%           & 4    & Time                                                          & description size                                                      & description size                                                  \\ \hline
%           & 5    & NA                                                            & Time days                                                             & Time days                                                         \\ \hline
% OpenOffice & 1    & Comment text                                                  & Comment text                                                          & Comment text                                                      \\ \hline
%           & 2    & Last status                                                   & Description text                                                      & Description text                                                  \\ \hline
%           & 3    & NA                                                            & fixer experience                                                      & fixer experience                                                  \\ \hline
%           & 4    & NA                                                            & Comment size                                                          & Comment size                                                      \\ \hline
%           & 5    & NA                                                            & Time days                                                             & Time days                                                         \\ \hline
% \end{tabular}
% \end{table}








% \definecolor{summary_color}{rgb}{0.7, 0.75, 0.71}

% \newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary of RQ~\thetcbcounter},enhanced,drop shadow={black!50!white},
%   coltitle=black,
%   top=0.3in,
%   attach boxed title to top left=
%   {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
%   boxed title style={size=small,colback=pink},#1}
  
% \begin{summary}[boxed title style={colback=summary_color}]
% The existing work to predict reopened bug reports is based on only 3 projects and out of them 2 projects (i.e., Apache and OpenOffice) have bug reports with data leak issues. When removing the bug reports with data leak issue, we could replicate the reopened bug prediction model performance findings in only 2 out of 3 projects (i.e., Eclipse and Openoffice). We also were able to replicate top most important features in predicting reopened bug reports in 2 out of 3 projects (i.e., Eclipse and OpenOffice) after removing the bug reports with data leak issues. We conclude that, the prior studies on reopened bug prediction are only based on effectively 2 projects, therefore there is a need to revisit reopened bug prediction study on a larger dataset.
% \end{summary}



==> Results.tex <==
TODO RESULTS


==> not_used_Methodology.tex <==
\subsection{RQ1: Do the prior results remain consistent when the data leak is addressed?}
\textbf{\textit{Motivation:}} We revisited Shihab’s reopened bug prediction work. we analyzed their datasets and we found that some of the bug reports contained the last status feature as “reopened” in projects Apache and OpenOffice. However, we did not find any such flawed bug reports in the Eclipse project. This indicates a data leak problem where the model is trying to predict reopened bug reports when the last status was already reopened. Finding the bug reports which were used for analysis is difficult as the dataset does not have the bug id. It is almost impossible to find the exact bugs, we had to apply search criteria such as bug reporter and bug component from the dataset to trace the exact bug report in Bugzilla.\\
We investigated the data leak in the dataset of three projects studied by Shihab et al. (i.e. Apache, Eclipse, and Open Office). We found that overall 80.6\% (745/924) of the reopened bug reports have the last status as “reopened” and 0.04\% (517/13400) non reopened bug reports have the last status as “Reopened” in the Apache project. 0.003\% (39/10569) reopened bug reports have the last status as either ``Reopened\textunderscore Fixed'', ``Reopened\textunderscore later'', ``Reopened\textunderscore Invalid'', ``Reopened\textunderscore wontfix'' and 0.002\% (65/29600) of non reopened bug reports have the last status as either of ``Reopened\textunderscore later'', ``Reopened\textunderscore duplicate'', ``Reopened\textunderscore remind'', ``Reopened\textunderscore invalid'', and ``Reopened\textunderscore wontfix'' in OpenOffice project. We did not find any such flawed bug reports in the Eclipse project.\\
We identified the data leak in Shihab’s dataset, we remove all the bug reports which have the last status as ``reopened'', We investigate if the performance of bug prediction models falls when we remove the flawed bug reports. Shihab et al. found that comment text is the most important feature when predicting reopened bug reports in Eclipse as well as Open Office projects. Whereas, the last status is the most important feature in predicting reopened bug reports. We investigate if these findings still hold after removing the flawed bug reports.

% link - https://tex.stackexchange.com/questions/48632/underscores-in-words-text

\textbf{\textit{Approach:}} We manually searched in Bugzilla about the bugs with criteria such as reporter names, components, and hardware as the bug id is not provided in the Emad’s bug dataset. We tracked down some of the bugs based on these search criteria. Some of the searches result in multiple bug reports, we had to study all of them manually, and based on closing month or resolved month or dates we need to identify matching bug reports. This is a challenging task as not all searches result in the exact mapping of bug reports with the dataset. However, we were able to identify many such bug reports which were present in the dataset. For example, in Figure \ref{fig_flawed_bug_report} the bug report below shows an Apache bug report that was labeled as ``reopened'' in its last status for predicting this bug as reopened. 

\begin{figure}
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.9\textwidth]{Figures/bugzilla_apache_953.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{Flawed Apache bug report with last status as reopened}
\label{fig_flawed_bug_report}       % Give a unique label
\end{figure}

We remove all the bug reports from the analysis which have last status as ``Reopened'', and we call this as reduced dataset. We implement the reopened bug prediction model. We execute the prediction model on two type of datasets i.e., whole dataset and reduced dataset. We use the JIRA dataset for our analysis. We use the same classifier (i.e. Decision Tree) as used by Shihab. We use SMOTE to address class imbalance problems. We also use Grid Search based hyperparameter tuning to improve the performance of the bug prediction model. Shihab used top node analysis for computing feature importance. However, we do apply the latest techniques for feature importance such as permutation feature importance, by computing feature importance for each permutation, and then ranking these features based on the Sk\textunderscore esd test. We also compare our feature importance results with those shared by Shihab. They compute the important features using top node analysis. They consider a feature as most important if it is always the root node. The other important features are on nodes with level 1.  As they go down the levels of the tree, the features become less important. To compare our results with their results. We use their top node analysis results to get top 5 important features. We select a feature as most important if its occurrence is maximum at the root node. We then select the next important feature with the second highest count on the root node and so on. If all the features on root node are selected then we select the feature with the most occurrence on level 1 nodes. If root node and level 1 nodes features are selected, then we don't select any other feature as they don't provide features on level 2 and subsequent levels on the tree. We then generate a table to compare our results with the results of Shihab's paper.

\begin{figure}
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.9\textwidth]{Figures/last_status_project1.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{Distribution plot of leaked feature from Shihab’s data}
\label{fig_distribution_plot_last_status_reopened}       % Give a unique label
\end{figure}

\begin{figure}
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=1.2\textwidth]{Figures/plot_Emad_all_vs_reduced_AUC.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{Reopened bug Prediction AUC for All vs reduced dataset}
\label{fig_AUC_all_vs_reduced}       % Give a unique label
\end{figure}

\textbf{\textit{Results:}} \textbf{80.62\% of the reopened bug reports in the Apache project and 0.36\% of the reopened bug reports in the OpenOffice project have data leak issues.}
We investigated the Shihab's dataset and we observe that 80.62\% (745/924) Reopened bug reports have the last status as ``Reopened'' and 3.85\% of the non reopened bug reports have the last status as ``Reopened''. We also observe that in OpenOffice project 0.36\% (39/10589) reopened bug reports have the last status as ``Reopened'' and 0.21\% (65/29600) of the non reopened bug reports have the last status as ``Reopened'', Whereas, we did not find any flawed bug report in Eclipse project. This suggests a Reopened event already occurred while predicting reopened bug reports, which leads to data leak. Figure \ref{fig_distribution_plot_last_status_reopened} shows the number of bug reports with the last status as Reopened in the Apache as well as OpenOffice projects. 

\textbf{AUC drops by 7.11\% when flawed bug reports are removed.} We remove the flawed bug reports from the analysis and we recompute the performance of the prediction model. We observe that the maximum drop in AUC of 7.11\% is reported in the Apache project. We did not observe any substantial change in the performance of OpenOffice project. Figure \ref{fig_AUC_all_vs_reduced} shows the AUC for various projects in all data as well as in the reduced dataset. We can see that for project Apache the new AUC is substantially less than the all data AUC without removing flawed bug reports.\\
Table \ref{table_reduced_vs_all} shows the performance of the reopened bug prediction model for all data vs reduced data. 
We observe that for the Apache project the precision of Reopened bug report prediction dropped by 43.02\% (38.4/67.4) and recall for of Reopened bug prediction dropped by 24.63\% (56.9/75.5) and F1 score dropped by 38.64\% (43.5/70.9). The AUC dropped by 7.11\% (87.5/94.2). The accuracy slightly improved by 1.97\%. There was no substantial change in performance metrics for prediction of non reopened bug reports. 

\textbf{Description text is the most important feature in the prediction of reopened bug reports in the Apache project.}
We observed that in Apache project the performance dropped significantly after removal of flawed bug reports. This also reflects in the analysis of the most important feature study in the Apache project, where we find that description text is the most important instead of Last status as discussed in Shihab's study.\\
Table \ref{table_feature_importance_RQ1} shows the most important features for three different scenarios i.e., Shared by Shihab, all data feature importance, reduced data feature importance. We see that in Apache and OpenOffice projects the top 2 important features in Shihab's paper include the last status. This can be due to the faulty behavior of this feature as we have seen that ``Last status'' feature has data leak issue. In our study we found that description text is important feature instead of Last status. For the Eclipse project we match the top 2 features by Shihab. The third feature as per the top node analysis study is Severity changed whereas we found that priority is the third most important feature. For Apache, we exactly match 2 features with their study with the order of importance. If we ignore importance order then we match 3 features in 5 most important features. For OpenOffice, They only provide 2 important features i.e., ``comment text'' and ``Last status'', we also found that ``comment text'' is the most important feature in OpenOffice dataset. Shihab et al. found in their study that last status and the comment text are the most important features in predicting reopened bug reports. Whereas we identify comments text as well as description text to be most important features in the reopened bug prediction in 3 Bugzilla projects (Apache, Eclipse and OpenOffice). 




% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\label{table_reduced_vs_all}
\caption{Model performance all data vs reduced dataset}
\Rotatebox{90}{%
\begin{tabular}{|l|l|r|r|r|r|r|r|r|r|}
\hline
{\color[HTML]{333333} Project Name} & Type of dataset                & \multicolumn{1}{l|}{{\color[HTML]{333333} Precision R}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Recall R}} & \multicolumn{1}{l|}{{\color[HTML]{333333} F1-Score R}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Precision NR}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Recall NR}} & \multicolumn{1}{l|}{{\color[HTML]{333333} F1-Score NR}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Average Accuracy}} & \multicolumn{1}{l|}{{\color[HTML]{333333} AUC}} \\ \hline
{\color[HTML]{333333} Apache}       & all data                       & {\color[HTML]{333333} 67.4 (0.55)}                      & {\color[HTML]{333333} 75.5 (0.29)}                   & {\color[HTML]{333333} 70.9 (0.17)}                     & {\color[HTML]{333333} 98.3 (0)}                          & {\color[HTML]{333333} 97.4 (0.01)}                    & {\color[HTML]{333333} 97.9 (0)}                         & {\color[HTML]{333333} 96 (0.01)}                             & {\color[HTML]{333333} 94.2 (0.04)}              \\ \hline
{\color[HTML]{333333} }             & {\color[HTML]{FF0000} reduced} & {\color[HTML]{FF0000} 38.4 (1.59)}                      & {\color[HTML]{FF0000} 56.9 (2)}                      & {\color[HTML]{FF0000} 43.5 (0.73)}                     & {\color[HTML]{FF0000} 99.3 (0)}                          & {\color[HTML]{FF0000} 98.5 (0.01)}                    & {\color[HTML]{FF0000} 98.9 (0)}                         & {\color[HTML]{FF0000} 97.9 (0.01)}                           & {\color[HTML]{FF0000} 87.5 (0.03)}              \\ \hline
{\color[HTML]{333333} Eclipse}      & all data                       & {\color[HTML]{333333} 62.2 (1.09)}                      & {\color[HTML]{333333} 69.7 (0.74)}                   & {\color[HTML]{333333} 65.2 (0.61)}                     & {\color[HTML]{333333} 94.1 (0.03)}                       & {\color[HTML]{333333} 91.5 (0.12)}                    & {\color[HTML]{333333} 92.6 (0.04)}                      & {\color[HTML]{333333} 88 (0.11)}                             & {\color[HTML]{333333} 84.5 (0.22)}              \\ \hline
{\color[HTML]{333333} }             & {\color[HTML]{FF0000} reduced} & {\color[HTML]{FF0000} 62.2 (1.09)}                      & {\color[HTML]{FF0000} 69.7 (0.74)}                   & {\color[HTML]{FF0000} 65.2 (0.61)}                     & {\color[HTML]{FF0000} 94.1 (0.03)}                       & {\color[HTML]{FF0000} 91.5 (0.12)}                    & {\color[HTML]{FF0000} 92.6 (0.04)}                      & {\color[HTML]{FF0000} 88 (0.11)}                             & {\color[HTML]{FF0000} 84.5 (0.22)}              \\ \hline
{\color[HTML]{333333} Openoffice}   & all data                       & {\color[HTML]{333333} 75.5 (0.21)}                      & {\color[HTML]{333333} 80.9 (1.91)}                   & {\color[HTML]{333333} 77.5 (0.73)}                     & {\color[HTML]{333333} 93.2 (0.18)}                       & {\color[HTML]{333333} 90.6 (0.07)}                    & {\color[HTML]{333333} 91.8 (0.05)}                      & {\color[HTML]{333333} 88 (0.11)}                             & {\color[HTML]{333333} 91.9 (0.19)}              \\ \hline
{\color[HTML]{333333} }             & {\color[HTML]{FF0000} reduced} & {\color[HTML]{FF0000} 75.4 (0.21)}                      & {\color[HTML]{FF0000} 80.7 (2.01)}                   & {\color[HTML]{FF0000} 77.3 (0.75)}                     & {\color[HTML]{FF0000} 93.2 (0.19)}                       & {\color[HTML]{FF0000} 90.5 (0.07)}                    & {\color[HTML]{FF0000} 91.7 (0.04)}                      & {\color[HTML]{FF0000} 88 (0.11)}                             & {\color[HTML]{FF0000} 92 (0.18)}                \\ \hline
\end{tabular}
}%
\end{table}




% \begin{table}[]
% \caption{Statistical significance: * p < 0.05, ** p < 0.01, *** p < 0.001}
% \Rotatebox{90}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l}
% \cline{1-9}
% Project Name    & Ratio Precision R & \begin{tabular}[c]{@{}l@{}}Ratio Recall\\ Reopened\end{tabular} & Ratio F1-Score R & Ratio Precision NR & Ratio Recall NR & Ratio F1-Score NR & Ratio Average Accuracy & Ratio AUC        &  \\ \cline{1-9}
% \textbf{Apache} & \textbf{0.57***}  & \textbf{0.75***}                                                & \textbf{0.61***} & 1.01***            & 1.01***         & 1.01***           & 1.02***                & \textbf{0.93***} &  \\ \cline{1-9}
% Eclipse         & 1                 & 1                                                               & 1                & 1                  & 1               & 1                 & 1                      & 1                &  \\ \cline{1-9}
% OpenOffice      & 0.99              & 0.99                                                            & 0.99             & 1                  & 0.99            & 0.99              & 1                      & 1                &  \\ \cline{1-9}
% \end{tabular}
% }%
% \end{table}

\begin{table}[]
\caption{Ratio of performance, where Statistical significance: * p < 0.05, ** p < 0.01, *** p < 0.001}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l}
\cline{1-9}
Project Name    & \begin{tabular}[c]{@{}l@{}}Ratio\\  Precision\\  R\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio\\  Recall\\ Reopened\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio\\  F1-Score R\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio \\ Precision NR\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio \\ Recall NR\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio \\ F1-Score \\ NR\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio\\  Average \\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ratio\\  AUC\end{tabular} &  \\ \cline{1-9}
\textbf{Apache} & \textbf{0.57***}                                                & \textbf{0.75***}                                                   & \textbf{0.61***}                                            & 1.01***                                                       & 1.01***                                                    & 1.01***                                                         & 1.02***                                                              & \textbf{0.93***}                                     &  \\ \cline{1-9}
Eclipse         & 1                                                               & 1                                                                  & 1                                                           & 1                                                             & 1                                                          & 1                                                               & 1                                                                    & 1                                                    &  \\ \cline{1-9}
OpenOffice      & 0.99                                                            & 0.99                                                               & 0.99                                                        & 1                                                             & 0.99                                                       & 0.99                                                            & 1                                                                    & 1                                                    &  \\ \cline{1-9}
\end{tabular}
\end{table}










\begin{table}[]
\label{table_feature_importance_RQ1}
\caption{Feature Rank in Shihab's data vs our data}
\begin{tabular}{lllll}
Project     & Rank & Shihab's feature   & Our Feature (reduced data) & Our feature (all data) \\
Apache      & 1    & Last status        & Description text           & Description text       \\
            & 2    & Description text   & Description Size           & Comments text          \\
            & 3    & Comment text       & Comments text              & Description size       \\
            & 4    & Number of comments & Number of comments         & Number of comments     \\
            & 5    & Month              & Time days                  & Number of files in fix \\
Eclipse     & 1    & Comment text       & Comment text               & Comment text           \\
            & 2    & Description text   & Description text           & Description text       \\
            & 3    & Severity changed   & Priority                   & Priority               \\
            & 4    & Time               & description size           & description size       \\
            & 5    & NA                 & Time days                  & Time days              \\
Open Office & 1    & Comment text       & Comment text               & Comment text           \\
            & 2    & Last status        & Description text           & Description text       \\
            & 3    & NA                 & fixer experience           & fixer experience       \\
            & 4    & NA                 & Comment size               & Comment size           \\
            & 5    & NA                 & Time days                  & Time days             
\end{tabular}
\end{table}

\definecolor{summary_color}{rgb}{0.7, 0.75, 0.71}

\newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary of RQ1},enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.3in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=pink},#1}
  
\begin{summary}[boxed title style={colback=summary_color}]
The existing reopened bug prediction study on Apache and OpenOffice is based on flawed dataset. When removing the flawed bug reports, the performance depreciates substantially. Also, the last status of the bug report is no longer the most important feature in prediction of the reopened bug report.
\end{summary}


%  RQ2 here 

\subsection{RQ2: Can we accurately predict whether a bug will be reopened using the more accurate dataset?}
\textbf{\textit{Motivation:}} Previous studies on predicting reopened bug reports relied on faulty datasets. We investigated that these collected bug reports from Bugzilla have data leak issues. In this RQ, We investigate the new dataset (i.e. JIRA bug reports). We carefully collected the dataset, we only considered the data fields which got updated before the first reopening of the bug reports, thereby preventing the data leak. We mapped all the features from the previous study [Shihab et al.]. There were 24 features in the Bugzilla dataset and in the JIRA dataset we collected  20 features. 4 features were not present in the JIRA dataset ( i.e. Platform, Severity, Number in the CC list, Severity changed). The bug reports consist of two text features (i.e. “comments” and “description”). We know that the old findings on the Bugzilla dataset are not valid anymore, so we investigate if we can accurately predict if a bug will be reopened with the newly collected dataset. Not all projects perform equally well on bug prediction models. Some projects have features that give very high AUC with a reopened bug prediction model, whereas some projects do not have a good reopened bug report prediction AUC. We investigate the following :
What are the good projects with high AUC?
What are the bad projects with low AUC?

\textbf{\textit{Approach:}}


==> replication_study.tex <==
\label{sec:replication}
In this section, we replicate a prior study by~\cite{shihab2013studying} on reopened bug prediction. We discuss the motivation, approach, and results of our replication study as follows.

\noindent \textbf{Motivation:}  Shihab et al. proposed a reopened bug prediction model using three projects (i.e., Apache, Eclipse, and OpenOffice) in the Bugzilla dataset and follow-up studies of reopened bug prediction used the same dataset. We replicate a prior study by Shihab et al. on reopened bug prediction for the following reasons. Since through our preliminary examination of the provided data by Shihab et al., we observe that some bug reports had their last status (an independent feature in training the model) as \textit{reopened}. Figure \ref{fig_data_leak_} shows a snapshot of the Apache project dataset, with the last status as \textit{reopened} in reopened and non-reopened bugs. This is a data leak issue~\citep{kaufman2012leakage}, which allows a reopened bug prediction model to predict if a bug will be reopened or not with knowing a bug's last status was \textit{reopened} already. The presence of such data leak in the studied projects might falsely inflate the performance of the reopened bug prediction models \citep{ribeiro2016should, kaufman2012leakage}. Therefore, we first wish to understand how many data points have the data leak issue and then evaluate if the findings presented in the study by Shihab et al. still hold after removing the data leak. %Such a replication is particularly important as the current state of the art reopened bug prediction model by~\citep{xia2015automatic} use the datasets provided by~\citep{shihab2013studying} to show the 

% since their proposed reopened bug prediction model is based on Bugzilla bugs, new bugs that are tracked in other ITS (e.g., JIRA and GitHub) are increasingly studied \citep{ma2017developers, zhang2018empirical, gyimesi2015characterization, zhou2017automated, herzig2013s}. In order to understand reopened bug prediction with newly available data sources, firstly we aim to replicate the study by Shihab et al.

\begin{figure}[!ht]
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.7\textwidth]{Figures/snapshot_data_leak.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{A snapshot of the data from the Apache project used by Shihab et al.}
\label{fig_data_leak_}       % Give a unique label
\end{figure}

Moreover, the study by Shihab et al. was conducted 8 years ago (i.e., in 2013). Several experimental components that they used in their pipeline to build a reopened bug prediction model have since then been shown to be not as effective when building a prediction model. Therefore, we replicate their study on their same projects (after removing the bugs with data leak), using an updated prediction pipeline that employs robust experimental components to build a reopened bug prediction model. For instance, Shihab et al. built a Decision Tree classifier without tuning the hyperparameters. However, several recent studies have shown that tuning the hyperparameters of a Decision Tree classifier is pivotal to ensure its optimal performance and interpretation~\citep{fu2016tuning,tantithamthavorn2018impact}. Furthermore, Shihab et al. used a class re-weighting and re-sampling strategy to deal with the class imbalance issue that is present in the projects. However, several recent studies have shown SMOTE to be a more effective method for class re-balancing~\citep{tantithamthavorn2018impact,agrawal2018better}. %


Finally, we choose to replicate the study by Shihab et al. in particular for two key reasons. First, the study by Shihab et al. is the first study that investigates the problem of reopened bug prediction at a large scale. The findings of the reopened bugs observed by Shihab et al. have since been used in several prior studies \citep{xia2015elblocker, xia2015automatic, le2015should, xia2017effective, an2018empirical}. Second, the current state of the art reopened bug prediction model by~\cite{xia2015automatic} uses both the dataset and results provided by Shihab et al. to demonstrate the efficiency of their approach. Therefore, it is pivotal that we replicate the study by Shihab et al. after addressing the aforementioned issues, to examine if their findings still hold, since the study by Shihab et al., might impact the findings of follow-up studies.\\

\noindent \textbf{Approach:} To replicate the study by Shihab et al. and analyze the impact of data leak and the outdated prediction pipeline on predicting reopened bugs, we first collect the projects provided by Shihab et al. (i.e., bug reports from Eclipse, Apache, and OpenOffice projects). We then replicate their study with an updated prediction pipeline (that we detail below). We do so by firstly building a reopened bug prediction model on the projects with all bug reports including those that exhibit data leak (i.e., the bug reports that have \textit{reopened} as their last status before getting closed). We label this dataset as ``all data''. We then compare the performance of the reopened bug prediction model that we built against the performance scores reported by Shihab et al. to examine if their results could be replicated (and possibly improved) with a more robust prediction pipeline that we employ. Furthermore, we examine if our constructed reopened bug prediction model can identify the same top features that Shihab et al. found to be most important (i.e., the feature importance) in identifying whether a bug report will get reopened.

Next, to study the impact of the data leak, we remove the bug reports that have their last status as \textit{reopened} and label the remaining bugs as ``refined data''. Following which, we construct a reopened bug prediction model with a more robust prediction pipeline similar to the previous step. We then compare the performance of our reopened bug prediction model constructed on ``refined data'' to that of the model constructed on ``all data'' and the results reported by Shihab et al. A significant drop in performance for our constructed reopened bug prediction model on the ``refined data" would indicate the impact of data leak on the obtained results and vice versa. Finally, we also compute the two most important features that help our reopened bug prediction model constructed on ``refined data'' in identifying whether a bug report would be reopened or not. We do so to observe if the removal of data leak in the project impacts the insights obtained from a reopened bug prediction model. 

Figure \ref{fig_Replication_approach} shows the workflow of replicating the reopened bug prediction model. We outline the steps that we follow to remove the data leak and construct the reopened bug prediction model with robust experimental components.

\begin{figure}[!ht]
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.7\columnwidth]{Figures/Replication_approach.pdf}
% figures can also be resized by adding to the include graphics command as follows
% \includegraphics[width=1.0\textwidth]{example.eps}
% figure caption is below the figure
\caption{Replicating reopened bug prediction workflow.}
\label{fig_Replication_approach}       % Give a unique label
\end{figure}

%  indent a paragraph 
% https://tex.stackexchange.com/questions/35933/indenting-a-whole-paragraph
\begin{quote}
\noindent\textbf{Step 1: Data leak removal.} We used a simple strategy to remove the bug reports that exhibit data leak from the studied projects. We analyzed the last status feature of the bugs in the dataset and removed the bug reports where the last status feature was \textit{reopened}. We removed all flawed bug reports from ``all data'' to obtain the ``refined data''.

\noindent\textbf{Step 2: Feature encoding.} We encoded the categorical features in the dataset using one-hot feature encoding to transform categorical features present in the dataset into numeric features to be used as an input to train the classifier \citep{zheng2018feature}. We employ one-hot feature encoding as opposed to simply converting the categorical features to numeric features as Shihab et al. We do so as~\cite{cerda2018similarity} stated that one-hot feature encoding is one of the latest and more widely used categorical feature encoding procedure. One-hot encoding creates a separate boolean column for each category of the categorical features. These columns are then passed along with the other numeric columns to the next step. 
%(i.e., reporter name, fixer name, component, platform, last status, and weekday)

\noindent\textbf{Step 3: Model construction.} In this step, we perform the following substeps:

\noindent\textbf{Step 3.1 Splitting dataset into training/testing sets.} We split the dataset into training and testing sets using 10-times-stratified 10-fold cross-validation as opposed to 10-times 10-fold cross-validation used by Shihab et al. In stratified 10-fold cross-validation, the whole dataset is split into 10 folds in such a way that each fold contains the same percentage of all class labels as in the overall dataset. Each fold is then used to test the model performance and the remaining 9 folds are used for training the model. We repeat this process 10 times. Therefore, for each iteration 10 performance and feature importance measures are generated and overall 100 performance and feature importance measures are generated on each studied project. For more details of the stratified k-fold cross-validation please refer to \cite{zeng2019automatic}. We choose 10-times-stratified-10-fold cross-validation in particular because our studied dataset is imbalanced, and stratified k-fold cross-validation helps preserve the original class distribution of the data \citep{he2013imbalanced,arellano2019epidemiological}. 
%Stratified k-fold cross-validation preserves the percentage of samples for each class label \citep{}.


\noindent\textbf{Step 3.2 Handling class imbalance.} Since the dataset for predicting reopened bugs is imbalanced (i.e., fewer reopened bugs as compared to non-reopened bugs), we used the SMOTE technique to rebalance the training dataset \citep{malhotra2017empirical}. SMOTE is an oversampling approach in which the minority class is over-sampled by generating synthetic samples \citep{chawla2002smote}. Shihab et al. used class re-weighting and a re-sampling strategy to deal with the class imbalance present in the dataset. However, we choose SMOTE for handling class imbalance as recent studies show that SMOTE is a more effective method for class re-balancing~\citep{tantithamthavorn2018impact,agrawal2018better}.

\noindent\textbf{Step 3.3 Training the classifier.} To build our reopened bug prediction model, we construct a classifier on the ``all data'' and ``refined data''. In our replication study, we used the same classifier (i.e., Decision Tree classifier) as used by Shihab et al. to construct the reopened bug prediction model.

\noindent\textbf{Step 3.4: Tuning the hyperparameters of the classifier.} We used the grid search \citep{sklearn_website_grid_search} based hyperparameters tuning to optimize the performance of the classifier. Grid search exhaustively considers all combinations of parameter values used to train the classifier and chooses the parameter that yields the best performance (we use AUC) for the constructed reopened bug prediction model.
Shihab et al. used a Decision Tree classifier without tuning the hyperparameters to build their reopened bug prediction model. However, several recent studies have shown that tuning the hyperparameters of a Decision Tree classifier is pivotal to ensure its optimal performance and interpretation~\citep{fu2016tuning,tantithamthavorn2018impact}. In our replication, we ensure that the hyperparameters used by Shihab~et~al. is encompassed in the grid that we use to tune our reopened bug prediction model. The hyperparameters that we tune for our Decision Tree classifier and their ranges as follows: 1) The minimum samples in a leaf node ranges from 1 to 12. 2) Criterion for measuring the quality of split is either gini or entropy. 3) Complexity parameter for minimal cost-complexity pruning ranges from 0 to 0.25.

%in our replication study, we used both the model parameter values used by Shihab et al. and default parameter values in WEKA (that was used by Shihab et al. to construct the model) as the range of hyperparameters. For example, Shihab et al. set the minimum node size of the tree as 10, we also considered this value in our hyperparameters range.

\noindent\textbf{Step 4: Model performance evaluation.} In this step, we used the same performance measures that Shihab~et~al. used to measure the performance of the constructed reopened bug prediction models. We do so to ensure that we can compare our obtained results to results reported in their study. They used F1-score-R and F1-score-NR for predicting F1-measure for reopened and non-reopened bugs, respectively. In our study, in addition to these performance measures, we also use AUC (Area Under the receiver operating characteristic Curve). We do so as several prior studies state that AUC is a robust measure that is sensitive to class distribution of the dataset \citep{rajbahadur2017impact, rajbahadur2019impact,ghotra2017large,lessmann2008benchmarking}. For each iteration of the 10-times-stratified-10-fold cross-validation we generate all the aforementioned performance measures. Finally, we compute the mean of the performance values across all the iteration, which is the same as Shihab~et~al.

%select the performance measures used to measure the performance of the constructed reopened bug prediction model. We The permutation feature importance method is based on repeated permutations of the outcome vector to estimate the distribution of measured importance for each feature \citep{altmann2010permutation}.

\noindent\textbf{Step 5: Ranking important features.} To generate the feature importance in predicting the reopened bugs, we used the permutation feature importance method \citep{altmann2010permutation}. We use the permutation feature importance method over the top node analysis used by Shihab et al. for the following reasons. First, Shihab~et~al. compute the feature importance ranks on re-balanced datasets. Second, the results of top node analysis can be biased since Decision Tree favors categorical features \citep{altmann2010permutation}. To avoid these shortcomings, we use a permutation feature importance method. The permutation feature importance method works as follows. First, we compute the performance of reopened bug prediction model. We then randomly permute the values of each feature at a time and compute the model's performance. We do so to note how much performance drop does permuting a feature encounters when compared to the model built on all the features whose values are not permuted. A larger drop in performance due to a permutation of a feature's value signifies the higher importance of that feature. 

For computing the feature importance ranks, we use the dataset as it is to train the classifier (i.e., we do not use SMOTE in feature importance analysis). We do so as \cite{tantithamthavorn2018impact} find that using class re-balancing techniques when computing feature importance ranks results may lead to wrong features being considered as the important features. After this step for each iteration of training data, feature importance scores are obtained for each feature. More details of the working of permutation feature importance method can be found in \cite{rajbahadur2017impact}. After generating the feature importance score, we compute the features importance ranks using Scott-Knott ESD test \citep{tantithamthavorn2016empirical}. These ranks determine the order of importance of features in predicting the reopened bugs. 
%Finally, as~\cite{altmann2010permutation} shows performed the top node analysis to rank the important features in predicting the reopened bugs. We used the permutation feature importance method to generate feature importance as it has been proven that if classifiers are categorical (i.e., decision tree) they are biased in favor of features with more categories and the permutation importance method can correct feature importance bias \citep{altmann2010permutation}.\hl{I checked before this point}

\end{quote}

Finally, we compare the model performance trained on ``all data'' vs ``refined data''. To measure the difference between the performance distributions of models trained on these two datasets, we use a Wilcoxon signed-rank test \citep{wilcoxon1946individual}. If the p-value of the Wilcoxon test between the two distributions is less than 0.05 we conclude that the two distributions are significantly different. Also, to quantify the extent of difference in the performance of models trained on ``all data'' and ``refined data'', we use Cohen's \textit{d} effect size test \citep{cohen1988statistical}. We used the same threshold values such as, $|$d$|\leqslant$0.2 : negligible (N), $|$d$|\leqslant$0.5 : small (S), $|$d$|\leqslant$0.8 : medium (M), $|$d$|>$0.8 : large (L) for measuring the effect size as used by prior studies \citep{rajbahadur2017impact, wilcox2011measuring, sullivan2012using}.

\noindent \textbf{Results: We are able to replicate (and slightly improve) the performance scores reported by Shihab et al. with our reopened bug prediction model on two out of three studied projects. However, on the OpenOffice project, even with an updated reopened bug prediction pipeline, we observe a slightly lower performance score for our constructed reopened bug prediction model than the study by Shihab et al.} Table~\ref{table:table_reduced_vs_all_RQ1} presents the performance scores reported by Shihab et al. and the performance scores obtained for our constructed reopened bug prediction models on ``all data''. From Table~\ref{table:table_reduced_vs_all_RQ1} we observe that for the OpenOffice project, the obtained F1-score-R for our reopened bug prediction model constructed on ``all data'' is 6.6.\% less than the F1-score-R reported by Shihab et al. Such a result is in spite of us using a more robust reopened bug prediction pipeline than the one employed by Shihab et al. Similarly, we also observe that the results obtained by our reopened bug prediction model built on ``all data'' yields 1.9\%, 2.9\% less F1-score-NR and accuracy respectively than the results reported by Shihab et al. In contrast, on Apache and Eclipse projects, we observe that our reopened bug prediction model yields better performance score across all the performance measures reported by Shihab et al. Such a result indicates that on these two projects the results are indeed replicable and the updated reopened bug prediction pipeline in fact helps improve the performance of the constructed reopened bug prediction models. In turn, on the OpenOffice project, we conclude that we were unable to replicate the results reported by Shihab et al.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[!ht]
% \caption{Performance of reopened bug prediction models reported by Shihab~et~al. and model trained on ``all data'' and ``reduced data''. The * indicates that model trained on ``reduced data'' has a p-value for the Wilcoxon signed-rank test less than 0.05 when compared to model trained on ``all data''. The value inside the parentheses indicates the magnitude of Cohen's \textit{d} effect size between the performance of models trained on ``all data'' and ``reduced data''.}
% \label{table:table_reduced_vs_all_RQ1}
% \begin{tabular}{|l|l|r|r|r|r|}
% \hline
% \textbf{Project name}                & \begin{tabular}[c]{@{}l@{}}\textbf{Type of} \\ \textbf{dataset}\end{tabular} & \multicolumn{1}{l|}{\textbf{F1-score-R}}                        & \multicolumn{1}{l|}{\textbf{F1-score-NR}}                        & \multicolumn{1}{l|}{\textbf{Accuracy}}                           & \multicolumn{1}{l|}{\textbf{AUC}}                               \\ \hline
% \multirow{3}{*}{Apache}     & Shihab et al.                                              & 67.2                                                   & 96.7                                                    & 94                                                      & -                                                      \\ \cline{2-6} 
%                             & All data                                                   & 70.9                                                   & 97.8                                                    & 95.9                                                    & 95                                                     \\ \cline{2-6} 
%                             & Reduced data                                               & \begin{tabular}[c]{@{}r@{}}46.5 \\ (2.8 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}98.8 \\ (-1.7 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}97.9 \\ (-1.7 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}87.4 \\ (1.8 L*)\end{tabular} \\ \hline
% \multirow{3}{*}{Eclipse}    & Shihab et al.                                              & 59.4                                                   & 90.2                                                    & 84.2                                                    & -                                                      \\ \cline{2-6} 
%                             & All data                                                   & 63.6                                                   & 92.4                                                    & 87.4                                                    & 83.8                                                   \\ \cline{2-6} 
%                             & Reduced data                                               & -                                                      & -                                                       & -                                                       & -                                                      \\ \hline
% \multirow{3}{*}{OpenOffice} & Shihab et al.                                              & 83.6                                                   & 93.6                                                    & 90.8                                                    & -                                                      \\ \cline{2-6} 
%                             & All data                                                   & 77                                                     & 91.7                                                    & 87.9                                                    & 92.3                                                   \\ \cline{2-6} 
%                             & Reduced data                                               & \begin{tabular}[c]{@{}r@{}}77.7 \\ (-0.1 N)\end{tabular} & \begin{tabular}[c]{@{}r@{}}91.9 \\ (-0.1 N)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}88.1 \\ (-0.1 N)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}92.5 \\ (-0.1 N)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}






% %%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\caption{Performance of reopened bug prediction models reported by Shihab~et~al. and model trained on ``all data'' and ``refined data''. The * indicates that model trained on ``refined data'' has a p-value for the Wilcoxon signed-rank test less than 0.05 when compared to model trained on ``all data''. The value inside the parentheses indicates the magnitude of Cohen's \textit{d} effect size between the performance of models trained on ``all data'' and ``refined data''.}
\label{table:table_reduced_vs_all_RQ1}
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Project\\ name\end{tabular}}         & \textbf{\begin{tabular}[c]{@{}l@{}}Type of \\ dataset\end{tabular}} & \multicolumn{1}{l|}{\textbf{F1-score-R}}               & \multicolumn{1}{l|}{\textbf{F1-score-NR}}               & \multicolumn{1}{l|}{\textbf{Accuracy}}                  & \multicolumn{1}{l|}{\textbf{AUC}}                      \\ \hline
\multirow{3}{*}{Apache}                                                 & Shihab et al.                                                       & 67.2                                                   & 96.7                                                    & 94                                                      & -                                                      \\ \cline{2-6} 
                                                                        & All data                                                            & 70.9                                                   & 97.8                                                    & 95.9                                                    & 95                                                     \\ \cline{2-6} 
                                                                        & \begin{tabular}[c]{@{}l@{}}Refined\\ data\end{tabular}              & \begin{tabular}[c]{@{}r@{}}46.5 \\ (2.8 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}98.8 \\ (-1.7 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}97.9 \\ (-1.7 L*)\end{tabular} & \begin{tabular}[c]{@{}r@{}}87.4 \\ (1.8 L*)\end{tabular} \\ \hline
\multirow{3}{*}{Eclipse}                                                & Shihab et al.                                                       & 59.4                                                   & 90.2                                                    & 84.2                                                    & -                                                      \\ \cline{2-6} 
                                                                        & All data                                                            & 63.6                                                   & 92.4                                                    & 87.4                                                    & 83.8                                                   \\ \cline{2-6} 
                                                                        & \begin{tabular}[c]{@{}l@{}}Refined\\ data\end{tabular}              & -                                                      & -                                                       & -                                                       & -                                                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Open-\\ Office\end{tabular}} & Shihab et al.                                                       & 83.6                                                   & 93.6                                                    & 90.8                                                    & -                                                      \\ \cline{2-6} 
                                                                        & All data                                                            & 77                                                     & 91.7                                                    & 87.9                                                    & 92.3                                                   \\ \cline{2-6} 
                                                                        & \begin{tabular}[c]{@{}l@{}}Refined\\ data\end{tabular}              & \begin{tabular}[c]{@{}r@{}}77.7 \\ (-0.1 N)\end{tabular} & \begin{tabular}[c]{@{}r@{}}91.9 \\ (-0.1 N)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}88.1 \\ (-0.1 N)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}92.5 \\ (-0.1 N)\end{tabular} \\ \hline
\end{tabular}
\end{table}





\textbf{We are able to replicate the feature importance ranks reported by Shihab et al. in all the three studied projects.} Table \ref{table:table_feature_importance_RQ1} shows the features reported at the top two ranks by our reopened bug prediction model and the study by Shihab et al. We observe a complete overlap between the features reported at the top two ranks by our reopened bug prediction model and the study by Shihab et al.% For the Apache project, Shihab et al. reported that the last status is the most important feature to predict reopened bugs, in our replication study we also observe that last status as reopened is the most important feature to predict reopened bugs. It also signifies that the feature with data leak issue is the most important feature in predicting the reopened bugs in the Apache project. Similarly, for Eclipse and OpenOffice project, we are able to replicate all the rank-1 and rank-2 important features.\atagra{Ankur STOP}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\caption{Top two important features reported by Shihab et al. and our models trained on ``all data'' and ``refined data''. The text inside parentheses indicates the category of the categorical features which is most important to predict reopened bugs}
\label{table:table_feature_importance_RQ1}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Project name}                & \textbf{Type of dataset} & \textbf{Rank-1}                                                            & \textbf{Rank-2}                                                              \\ \hline
\multirow{3}{*}{Apache}     & Shihab et al.   & Last status                                                       & Description text                                                    \\ \cline{2-4} 
                            & All data        & \begin{tabular}[c]{@{}l@{}}Last status \\ (reopened)\end{tabular} & Description text                                                    \\ \cline{2-4} 
                            & Refined data    & Description text                                                     & \begin{tabular}[c]{@{}l@{}}Last status \\ (discussion)\end{tabular} \\ \hline
\multirow{3}{*}{Eclipse}    & Shihab et al.   & Comment text                                                      & Description text                                                    \\ \cline{2-4} 
                            & All data        & Comment text                                                      & Description text                                                    \\ \cline{2-4} 
                            & Refined data    & -                                                                 & -                                                                   \\ \hline
\multirow{3}{*}{OpenOffice} & Shihab et al.   & Comment text                                                      & Last status                                                         \\ \cline{2-4} 
                            & All data        & Comment text                                                      & Last status                                                         \\ \cline{2-4} 
                            & Refined data    & Comment text                                                      & Last status                                                         \\ \hline
\end{tabular}
\end{table}


% GOPI PREVIOUS
% \textbf{We further observe that, our reopened bug prediction model finds results in different feature importance ranks than the ones reported by~\cite{shihab2013studying} on two of the three studied projects.} Table~\ref{tabel:feature_importance_analysis} presents the features reported at the top two ranks by our reopened bug prediction model and the study by~\cite{shihab2013studying}. For both Apache and OpenOffice projects we observe that atleast one of the features reported at the top two ranks vary (for Apache project, the feature importance ranks of both the features reported at the top two ranks vary). However, for Eclipse project, our reopened bug prediction model yields the same feature importance ranks as the ones reported by~\cite{shihab2013studying}.




%On Apache and Eclipse datasets, our constructed reopened bug prediction models, exhibited slightly improved performance scores than the performance scores reported by~\cite{shihab2013studying}.


%we were not able to replicate Shihab et al.'s study performance in 1 out of 3 projects (i.e., OpenOffice) using the ``all data'' even with an updated reopened bug prediction pipeline. We compared the \textit{F1-score} and \textit{accuracy} of Shihab et al. work with the obtained results from our replication using the updated reopened bug prediction pipeline. We were able to achieve better performance in the Apache and Eclipse project. However, for the OpenOffice project, we did not achieve the same performance as achieved by Shihab et al. while replicating the reopened bug prediction model performance with the ``all data'' (i.e., without removing the flawed bugs). Table \ref{table:table_reduced_vs_all_RQ1} shows the comparison of the performance of the replication study with the performance reported by Shihab et al.


% previous table
% \begin{table}[!ht]
% \caption{Comparing model performance for different datasets\gopi{caption needs to change. In the paranthessis dont include variance. Just P-values and effect size magnitude}\atagra{caption is changed}\atagra{issue with this as 1) we are comparing only on all data set and reduced dataset, if we give p-values here then Shihab et al. rows will be empty and all data rows will contain p-values, it will not be a symmetric table}}
% \label{table:table_reduced_vs_all_RQ1}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Project name                & Type of dataset & F1-score-R & F1-score-NR & Accuracy   & AUC       \\ \hline
% \multirow{3}{*}{Apache}     & Shihab et al.   & 67.2(0.07)  & 96.7(0.00)  & 94.0(0.00) & -         \\ \cline{2-6} 
%                             & All data        & 70.9(0.0)   & 97.8(0.0)   & 95.9(0.0)  & 95(0.0)   \\ \cline{2-6} 
%                             & Reduced data    & 46.5(0.01)  & 98.8(0.0)   & 97.9(0.0)  & 87.4(0.0) \\ \hline
% \multirow{3}{*}{Eclipse}    & Shihab et al.   & 59.4(0.55)  & 90.2(0.07)  & 84.2(0.15) & -         \\ \cline{2-6} 
%                             & All data        & 63.6(0.01)  & 92.4(0.0)   & 87.4(0.0)  & 83.8(0.0) \\ \cline{2-6} 
%                             & Reduced data    & -  & -   & -  & - \\ \hline
% \multirow{3}{*}{OpenOffice} & Shihab et al.   & 83.6(0.01)  & 93.6(0.00)  & 90.8(0.00) & -         \\ \cline{2-6} 
%                             & All data        & 77(0.01)    & 91.7(0.0)   & 87.9(0.0)  & 92.3(0.0) \\ \cline{2-6} 
%                             & Reduced data    & 77.7(0.01)  & 91.9(0.0)   & 88.1(0.0)  & 92.5(0.0) \\ \hline
% \end{tabular}
% \end{table}


%Shihab et al. reported the accuracy for the Apache and Eclipse projects as 94\% and 84.2\% respectively. However, our updated model achieved an accuracy of 95.9\% and 87.4\% for these two projects respectively. We improved the accuracy of the Apache project by 2\% and Eclipse project by 3.8\%. However, we did not achieve the same performance for the OpenOffice project as reported by Shihab et al. For example, Shihab et al. reported the accuracy for OpenOffice as 90.8\%, whereas we achieved an accuracy of 87.9\% in the Apache project, which is 3.2\% less than as reported by Shihab et al.

\textbf{We observe that among the three studied projects, the Apache project contains the most number of bug reports that exhibit data leak (i.e., 1,262 out of 14,324).} We find that bug reports in two out of the three studied projects (i.e., Apache and OpenOffice) exhibit data leak. Table~\ref{fig_distribution_plot_last_status_reopened} shows the number of bugs with the last status as \textit{reopened} in the Apache and the OpenOffice projects. From Table~\ref{fig_distribution_plot_last_status_reopened}, we observe that the Apache project exhibits a significantly more percentage of bug reports (8.8\%) that exhibit data leak in comparison to the OpenOffice project, which exhibits only 0.3\% (i.e., 104 out of 40,169) of bug reports that exhibit data leak. In particular, in the Apache project, 80.6\% (i.e., 745 out of the 924) bugs labeled as reopened have the last status as \textit{reopened}. 

% \begin{figure}[!ht]
% \centering
% % Use the relevant command to insert your figure file.
% % For example, with the graphicx package use
%   \includegraphics[width=0.9\textwidth]{Figures/last_status_project1.pdf}
% % figures can also be resized by adding to the include graphics command as follows
% % \includegraphics[width=1.0\textwidth]{example.eps}
% % figure caption is below the figure
% \caption{Distribution of bug reports that exhibit data leak in the projects studied by Shihab~et~al.}
% \label{fig_distribution_plot_last_status_reopened}       % Give a unique label
% \end{figure}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\caption{Distribution of bug reports that exhibit data leak in the projects studied by Shihab~et~al.}
\label{fig_distribution_plot_last_status_reopened}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Project name}       & \textbf{Type of bug} & \textbf{\begin{tabular}[c]{@{}l@{}}Last status \\ as \textit{reopened}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Last status as either\\ \textit{closed} or \textit{resolved}\end{tabular}} \\ \hline
\multirow{2}{*}{Apache}     & Reopened             & 745 (5.2\%)                                                                 & 179 (1.2\%)                                                                           \\ \cline{2-4} 
                            & Non-reopened         & 517 (3.6\%)                                                                 & 12883 (89.9\%)                                                                        \\ \hline
\multirow{2}{*}{OpenOffice} & Reopened             & 39 (0.1\%)                                                                  & 10530 (26.2\%)                                                                        \\ \cline{2-4} 
                            & Non-reopened         & 65 (0.2\%)                                                                  & 29535 (73.5\%)                                                                        \\ \hline
\end{tabular}
\end{table}


\textbf{Once we remove the data leak and construct a reopened bug prediction model on the Apache project, we observe up to a 20.7\% drop in performance across the studied performance measures compared to the results reported by Shihab et al.} Table~\ref{table:table_reduced_vs_all_RQ1} compares the performance of the reopened bug prediction model trained on the ``refined data'' (i.e., the projects without bug reports that exhibit data leak). From Table~\ref{table:table_reduced_vs_all_RQ1} we observe that on the Apache project, while the F1-score-R is negatively impacted, the F1-score-NR and accuracy slightly increase in comparison to the results reported by Shihab et al. Wilcoxon signed-rank test results show that the performance of model trained on Apache project significantly changes after removing the data leak affected bug reports from the analysis when compared to model trained on ``all data'' for Apache project. Also, Cohen's \textit{d} results show that the performance difference between models trained on ``all data'' and ``refined data'' is large for the Apache project. We assert that such a result is because, upon removal of bug reports that exhibit data leak from the project, the number of reopened bugs that remain in the project becomes extremely low. In turn, it biases the reopened bug prediction model to predict most bugs as non-reopened. Our assertion is further supported by noting the impact of data leak on the performance in terms of AUC between the reopened bug prediction model trained on ``all data'' vs ``refined data'' on the Apache project. We observe a 7.6\% drop in performance in terms of AUC which outlines the severe impact that a 8.8\% of data leak present in the Apache project. However, a similar impact does not exist for both OpenOffice (where the bug reports that exhibit data leak is negligible) and Eclipse (which does not contain bug reports that exhibit data leak).  

%\gopi{@Ankur:Change dataset to project everywhere. Make sure all numbers below 5 are mentioned as five, four, etc}\atagra{done at places where it was possible}

%\textbf{2 out of 3 studied projects (i.e., Apache and OpenOffice) have data leak issues and after removing the bugs with data leak issues, we were not able to replicate reopened bug prediction model performance in 1 project (i.e., Apache)} We investigated the Shihab et al. dataset and we observed that, in the Apache project, there are 8.8\% (i.e., 1,262 out of 14,324) bugs with a \textit{reopened} last status. More specifically, 80.6\% (i.e., 745 out of the 924) bugs labeled as reopened have the last status as \textit{reopened}. In these bugs, the last status before the first occurrence of bug reopening should not be \textit{reopened}. In addition, 3.9\% (i.e., 517 out of the 13,400) bugs labeled as non reopened have the last status as \textit{reopened}. In these bugs, the last status should not be \textit{reopened} because a bug labeled as non reopened can't have a reopened state. There were also some flawed bugs (i.e., \textit{last status} as \textit{reopened}) in OpenOffice project, but these bugs were negligible. For example, in the OpenOffice project, only 0.3\% (i.e., 104 out of 40,169) bugs have the last status as \textit{reopened}. More specifically, 0.4\% (i.e., 39 out of 10,569) bugs labeled as reopened have their last status as \textit{reopened} and 0.2\% (i.e., 65 out of 29,600) bugs labeled as non reopened have the last status as \textit{reopened}. However, we did not find any bug with the last status as \textit{reopened} in the Eclipse project. Figure \ref{fig_distribution_plot_last_status_reopened} shows the number of bugs with the last status as \textit{reopened} in the Apache and the OpenOffice projects.



%After removing the flawed bugs, we observed that the model performance drops in the Apache project. More specifically, \textit{fi-score R} dropped from 70.9\% to 46.5\%, that is a substantial drop of 34.4\%. Also, the AUC dropped from 95\% to 87.4\%, which is a 8\% drop in AUC. Table \ref{table:table_reduced_vs_all_RQ1} shows the performance of model with ``all data'' and ``reduced data''. Table \ref{table:p_value} shows the ratio of performance obtained by dividing the mean performance obtained by removing the flawed bugs to the mean performance achieved using all the bugs (i.e., including flawed bugs). In the Apache project, there is a significant change in all the performance measures (i.e., \textit{F1-score R}, \textit{F1-score NR}, \textit{accuracy}, and AUC) obtained after removing the flawed bugs, however, for the OpenOffice project, there is no significant change in any of the performance measure after removing the flawed bugs. 

% \begin{table}[!ht]
% \caption{Ratio of performance, where statistical significance: * p$<$0.05, ** p$<$0.01, *** p$<$0.001 \gopi{why is this a seperate table..merge this with the table above and use stars besides the values and p-value in the paranteheis. (just 0.05 level is good. Give effect size values)}}
% \label{table:p_value}
% \begin{tabular}{|l|r|r|r|r|}
% \hline
% Project name & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Ratio F1- \\ score-R\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Ratio F1-\\ score-NR\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Ratio \\ accuracy\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Ratio\\ AUC\end{tabular}} \\ \hline
% Apache       & 0.66***                                                                              & 1.01***                                                                              & 1.02***                                                                           & 0.92***                                                                     \\ \hline
% OpenOffice   & 1.01                                                                              & 1                                                                                 & 1                                                                              & 1                                                                        \\ \hline
% \end{tabular}
% \end{table}

\textbf{Furthermore, we observe that after removing bug reports that exhibit data leak, the obtained feature importance ranks of the reopened bug prediction model change.} From the Table~\ref{table:table_feature_importance_RQ1}, we observe that in the Apache project, which has a significant number of bug reports with data leak, the rank-1 and rank-2 features interchange their importance when using reopened bug prediction model trained on ``refined data'' instead of ``all data''. More specifically, in the Apache project, \textit{last status} as \textit{reopened} is the most important feature for the model trained on ``all data'' to predict reopened bugs and after removing bug reports with data leak, \textit{description text} becomes the most important feature to predict the reopened bugs. Whereas, in the OpenOffice project, which has a negligible percentage of bug reports with data leak, the reopened bug prediction model constructed on ``all data'' and ``refined data'' results in the same feature importance ranks. Such a result indicates that in addition to impacting the performance of the reopened bug prediction model, the data leak presented in the projects could also change the interpretation of the constructed reopened bug prediction model.

%\textbf{After handling the data leak and with an updated pipeline, we were able to achieve a 66.7\% overlap in rank-1 and 33.3\% overlap in rank-2 in feature importance analysis compared with Shihab et al. results.} Table \ref{table:table_feature_importance_RQ1} shows the rank-1 and rank-2 features found by Shihab et al. and computed by our replication study with ``reduced data''. In two projects (i.e., Eclipse and OpenOffice) we get the same feature as a rank-1 feature as found by Shihab et al. However, for the Apache project Shihab et al. found that rank-1 feature is \textit{last status}, whereas we observe that \textit{description text} is the rank-1 feature in the Apache project. Also, only in one out of three projects (i.e., Eclipse) we get the same feature as a rank-2 feature as found by Shihab et al. For the Apache project, Shihab et al. found that \textit{description text} is the rank-2 feature, whereas we observe that \textit{description size} is the rank-2 feature and For OpenOffice project, Shihab et al. found that \textit{last status} is the 
%rank-2 feature, whereas we observe that \textit{description text} is the rank-2 feature.


















% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% #########################




% #########################












% [boxsep=1pt,left=2pt,right=2pt,top=0pt,bottom=0pt]

\begin{summary_new}[left=8pt,right=8pt,top=10pt,bottom=10pt,boxed title style={colback=summary_color}]{\bfseries{Summary of replication study}}
After removing the bugs with data leak issues and updating the reopened bug prediction pipeline, we were able to replicate Shihab et al.'s work in only one out of three studied projects (i.e., Eclipse). In one project (i.e., OpenOffice) we did not achieve the same performance with a more robust reopened bug prediction pipeline, whereas in another project (i.e., Apache) we did not achieve the same performance after removing bugs with data leak issues. Such a result shows that the Shihab et al. study is not fully replicable and that both outdated experimental components and data leakage can severely impact the performance of a reopened bug prediction model. %The removal of bug reports with data leak issues from the Shihab et al.'s dataset leads to drop in the performance and change in feature importance of the reopened bug prediction model.


\end{summary_new}


% \h{make this a box}










% Notes 
%  \footnote{\url{https://machinelearningmastery.com/why-one-hot-encode-data-in-machine-learning/}}



% We wish to find if their original findings still hold once we address the data leak issues that we observed in two of their three studied projects.




